2018 Robotic Scene Segmentation Challenge

In 2015 we began a sub-challenge at the EndoVis workshop at MICCAI in Munich using endoscope images of ex-vivo tissue with automatically generated annotations from robot forward kinematics and instrument CAD models. However, the limited background variation and simple motion rendered the dataset uninformative in learning about which techniques would be suitable for segmentation in real surgery. In 2017, at the same workshop in Quebec we introduced the robotic instrument segmentation dataset with 10 teams participating in the challenge to perform binary, articulating parts and type segmentation of da Vinci instruments. This challenge included realistic instrument motion and more complex porcine tissue as background and was widely addressed with modifications on U-Nets and other popular CNN architectures. In 2018 we added to the complexity by introducing a set of anatomical objects and medical devices to the segmented classes. To avoid over-complicating the challenge, we continued with porcine data which is dramatically simpler than human tissue due to the lack of fatty tissue occluding many organs.

==> tex/discussion.tex <==
\subsection{Discussion and conclusions}

% lessons learned from data collection/annotation
Major takeways are that the volume of data is not close to sufficient for recognizing most anatomical classes reliably given the huge appearance variation that occurs due to fat, connective tissue and other occluding surfaces. 

% lessons learned from methods
%Aggregating all of the results together in Table \ref{tab:dataset_overall_results} shows a large disparity between some classes in the mean IoU scores. The instrument shaft is by far the most easily recognized class, with an average mean IoU of 0.738. The kidney parenchyma, the instrument claspers and wrist and the surgical clips all have mean IoU scores of approximately 0.5. The worst performing classes were the thread, needle and US probe. The thread and needle are small, thin structures which are often not detected by CNNs and also constitute a very small fraction of the training datapoints, particularly with respect to their surroundings, meaning trained networks may learn to ignore them. The US probe also only appears in 2 (CHECK THIS) datasets and has very similar texture to the da Vinci instruments. Several teams did not predict any correct pixels for this task (why was this...?)


